Investigating Transferability in Pretrained Language Models

How does language model pretraining help transfer learning? We consider a simple ablation technique for determining the impact of each pretrained layer on transfer task performance. This method, partial reinitialization, involves replacing different layers of a pretrained model with random weights, then finetuning the entire model on the transfer task and observing the change in performance. This technique reveals that in BERT, layers with high probing performance on downstream GLUE tasks are neither necessary nor sufficient for high accuracy on those tasks. Furthermore, the benefit of using pretrained parameters for a layer varies dramatically with finetuning dataset size: parameters that provide tremendous performance improvement when data is plentiful may provide negligible benefits in data-scarce settings. These results reveal the complexity of the transfer learning process, highlighting the limitations of methods that operate on frozen models or single data samples.

==> __latexindent_temp.tex <==
@article{matthews1975comparison,
  title={Comparison of the predicted and observed secondary structure of T4 phage lysozyme},
  author={Matthews, Brian W},
  journal={Biochimica et Biophysica Acta (BBA)-Protein Structure},
  volume={405},
  number={2},
  pages={442--451},
  year={1975},
  publisher={Elsevier}
}

==> header.tex <==
% %
% % File emnlp2020.tex
% %
% %% Based on the style files for ACL 2020, which were
% %% Based on the style files for ACL 2018, NAACL 2018/19, which were
% %% Based on the style files for ACL-2015, with some improvements
% %%  taken from the NAACL-2016 style
% %% Based on the style files for ACL-2014, which were, in turn,
% %% based on ACL-2013, ACL-2012, ACL-2011, ACL-2010, ACL-IJCNLP-2009,
% %% EACL-2009, IJCNLP-2008...
% %% Based on the style files for EACL 2006 by 
% %%e.agirre@ehu.es or Sergi.Balari@uab.es
% %% and that of ACL 08 by Joakim Nivre and Noah Smith

% \documentclass[11pt,a4paper]{article}
% \usepackage[hyperref]{emnlp2020}
% \usepackage{times}
% \usepackage{latexsym}
% \renewcommand{\UrlFont}{\ttfamily\small}

% % This is not strictly necessary, and may be commented out,
% % but it will improve the layout of the manuscript,
% % and will typically save some space.n
% \usepackage{microtype}

% \usepackage{booktabs} % To thicken table lines

% \usepackage{graphicx}

% \newcommand{\alex}[1]{\textcolor[rgb]{.9,0,0}{\bf [Alex: #1]}}
% \newcommand{\ndg}[1]{\textcolor[rgb]{.2,0,.8}{\bf [Noah: #1]}}
% % \newcommand{\alex}[1]{\textcolor[rgb]{.9,0,0}{}}
% % \newcommand{\ndg}[1]{\textcolor[rgb]{.2,0,.8}{}}


% \aclfinalcopy % Uncomment this line for the final submission
% \def\aclpaperid{***} %  Enter the acl Paper ID here

% %\setlength\titlebox{5cm}
% % You can expand the titlebox if you need extra space
% % to show all the authors. Please do not make the titlebox
% % smaller than 5cm (the original size); we will check this
% % in the camera-ready version and ask you to change it back.

% \newcommand\BibTeX{B\textsc{ib}\TeX}

==> related.tex <==
\label{sec:related}

Recent work on understanding the parameters of deep NLP models has centered on \emph{probing}, a methodology for determining whether certain infromation is present at different components of a neural network \citep{conneau2018you, hupkes2018visualisation, liu2019linguistic, tenney2019bert, goldberg2019assessing, tenney2019you,  hewitt2019structural} This work is closely connected to earlier work in neuroscience on neural decoding, which seeks the same goals for representations in the brain \citep{haxby2001distributed, kamitani2005decoding, harrison2009decoding}. But these studies stop short of connecting the existence and location of this information to its effects on finetuning.

% By design, such approaches are meant to uncover only knowledge that is \emph{manifest}, in that the representations are organized such that simple models like logistic regression can access them. However, there may still be \emph{latent knowledge} \citep{vokey1999implicit} learned during pretraining which requires a more complex model to leverage but yet which ultimately improves downstream performance.

In computer vision, a swath of recent work investigates how finetuning performance is affected by pretraining data and optimization strategies \citep{huh2016makes, ngiam2018domain, kornblith2019better}. By contrast, we investigate the specific products of the pretraining process, the learned parameters, which are the more direct source of transfer ability. 

In an NLP context, \citet{hao2019visualizing} analyze the effects of BERT pretraining on the finetuning loss landscape; however, their visualization method does not establish what characteristics of BERT are responsible for these effects.

Our work is most similar to a line of work in computer vision which uses selective reinitialization as a tool to explore the transferability of different layers in ImageNet-pretrained models \citep{yosinski2014transferable, raghu2019transfusion}. The closest parallel in NLP is a limited analysis study in \citet{radford2018improving}. However, these studies comingle important phenomena which we untangle, including: 1) task vs dataset size, 2) location vs quantity of layers, and 3) presence vs organization of layers.
